For high-dimensional hierarchical models, consider exchangeability of effects across covariates instead of across datasets

Hierarchical Bayesian methods enable information sharing across multiple related regression problems. While standard practice is to model regression parameters (effects) as (1) exchangeable across datasets and (2) correlated to differing degrees across covariates, we show that this approach exhibits poor statistical performance when the number of covariates exceeds the number of datasets. For instance, in statistical genetics, we might regress dozens of traits (defining datasets) for thousands of individuals (responses) on up to millions of genetic variants (covariates). When an analyst has more covariates than datasets, we argue that it is often more natural to instead model effects as (1) exchangeable across covariates and (2) correlated to differing degrees across datasets. To this end, we propose a hierarchical model expressing our alternative perspective. We devise an empirical Bayes estimator for learning the degree of correlation between datasets. We develop theory that demonstrates that our method outperforms the classic approach when the number of covariates dominates the number of datasets, and corroborate this result empirically on several high-dimensional multiple regression and classification problems.

==> related_work.tex <==
\subsection{Related work}\label{sec:related_work}
% Brown and Zidek
To our knowledge, the notion of exchangeability among covariate effects is essentially absent from the existing literature on hierarchical Bayesian regression.
Perhaps the only exception a brief contribution by \citet{brown1980adaptive}, and a single follow-up paper by \citet{haitovsky1987multivariate}.
However, as compared the present work, these two brief papers have far narrower scope in that both
(1) consider only the situation in which a single design matrix is shared across all datasets (or equivalently, for each data-point all $Q$ responses are observed) and
(2) include only theoretical (rather than empirical) evaluations.
Nonetheless, this early work provides an important starting point from which the present paper builds.

%\citet{brown1980adaptive} consider extensions of ridge regression \citep{hoerl1970ridge} applicable to multiple datasets.
%Though the paper makes only brief mention of Bayesian connections (their primary concern is frequentist comparison to maximum likelihood),
%their estimates resemble a special case of ours.
%Furthermore, they note in passing that their `result is implicitly in the work of \citet{lindley1972bayes} although not actually developed there', 
%but provide no further clarification.
%In a short follow-up paper, \citet{haitovsky1987multivariate} elaborates on this hierarchical Bayesian motivation.
%The primary focus of \citet{haitovsky1987multivariate} is a matrix normal prior that captures structure in effects across both datasets and covariates.
%Though this prior is not exchangeable across covariate effects in general, they note 
%that the special case of where effects are uncorrelated across different covariates satisfies the notion of exchangeability we advocate for here.
%Both \citet{brown1980adaptive} and \citet{haitovsky1987multivariate} consider 
%only situations in which the design matrices of all datasets are shared (i.e.\ $X^1=X^2=\dots=X^Q$) and neither include empirical evaluations.

Though notion of exchangeability among covariate effects is absent from existing work in statistical genetics,
multivariate normal priors of the form described in \Cref{sec:hierarchical_regression} have nevertheless been used to model the distribution of effects of DNA sequence changes (the covariates) on multiple related traits.
Existing work has used this model structure
to understand genetic similarities between traits \citep{lee2012estimation,bulik_finucane2015atlas}, 
to improve association mapping \citep{stephens2013unified,zhou2014efficient},
and to improve risk prediction \citep{maier2015joint,runcie2020megalmm}.
Our belief is that the historical basis of these methods provided a route to their development that obviated the need for the idea of exchangeability.
In particular, these ideas have their roots in mixed effects modeling in cattle breeding \citep{thompson1973estimation}, wherein the earlier notion of the genetic contribution of trait correlation (i.e.\ `genetic correlation' \citep{hazel1943genetic}) informs the covariance structure of random effects.
We suspect this older concept facilitated the intellectual leap to such priors without the need to first consider exchangeability among the effects of individual covariates.
Indeed, though `genetic correlation' is now commonly understood to describe the correlation of effects of DNA sequence changes on different traits \citep{bulik_finucane2015atlas}, its provenance predates even the first identification of DNA as the genetic material \citep{avery1944studies}.
Intriguingly, despite the long history and success of this class of models in statistical genetics, to our knowledge they have not previously been generalized to other contexts.
We suspect that the firm grounding of this approach in the widely accepted and context specific idea of genetic correlation may have served as a roadblock that obscured its possible generalization to other applications.

%Within the Bayesian community, some recent works have sought to leverage relatedness between high-dimensional regression problems.
%For example, \citet{navon2018capturing} describe an approach that captures `within group' variation in regression coefficients;
%however, their approach restricts to a narrower class of priors for which the effects remain exchangeable across datasets.
%\citet{deshpande2019simultaneous} consider similar patterns of sparsity across datasets, but do not allow for correlation in associated effects across datasets.

We discuss additional related work in \Cref{sec:additional_related_work}.

